A self-consistent refractive index model for fast simulation of free-electron lasers

Modern x-ray free-electron lasers (XFELs) produce x-ray pulses of exceptional transverse coherence. This is due largely to the process of optical guiding by which the radiation is both refractively guided by the bunched electron beam and gain guided by the preferential amplification of on-axis radiation. These effects may be summarized by an effective index of refraction, which has been used in the past to study the transverse dynamics of the FEL process with significant simplifications and approximations, but never fully self-consistently. We present here a self-consistent method for studying high gain FELs in the linear regime by approximating the FEL equations to second-order in the lateral displacement from the nominal electron beam axis. This is made possible by casting the FEL equations in the language of optical fibers with an appropriately chosen refractive index. We demonstrate that this approach is both fast and highly accurate, indicating that the most important FEL dynamics are inherently second-order. In its full form our method can capture the effects of transverse offsets in both the x-ray beam and the electron beam, making it a versatile tool for studying non-ideal effects in seeded FELs, regenerative amplifier XFELs, and even self-amplified spontaneous emission (SASE) FELs.

==> IntroArchive.tex <==

%this is not actually the first paragraph, just where I thought to start first 
The phenomenon of optical guiding is critical to the feasibility of modern x-ray free-electron lasers. It enables the long undulator lengths necessary to sustain sufficient power gain to reach saturation. It can generally be separated into two different effects: the first is gain guiding in which the gaussian nature of the electron beam causes on-axis radiation to be preferentially amplified relative to off-axis radiation. The second is refractive guiding analogous to the behavior of electromagnetic fields in optical fibers whereby the partially bunched electron beam acts as a dielectric medium with some non-vacuum permittivity. These effects are characterized by the imaginary and real parts of an effective refractive index, respectively. 

Many early treatments of optical guiding summarized the FEL physics using an effective index of refraction. This effective refractive index can be found by writing the FEL wave equation in the form of the paraxial wave equation in a dielectric waveguide (see e.g. \cite{marcuse2013})
\begin{equation}\label{eqn:dielectricwaveguideeqn}
    2ik_r\frac{\partial E}{\partial z} + \nabla_\perp^2E = k_r^2\left(1-n(r,z)^2\right)E
\end{equation}
In the language of \cite{prosnitz1981}, in a FEL with azimuthal symmetry this has the form
\begin{equation}\label{eqn:prosnitzindex}
    n(r,z) = 1 + \frac{1}{2}\frac{\omega_b(r,z)^2}{\omega^2}\left<\frac{e^{-i\psi}}{\gamma}\right>\frac{a_w}{\abs{a(r,z)}}
\end{equation}
where here $\omega_b(r,z)$ is the local electron plasma frequency, $\omega$ is the resonant radiation frequency, $\psi$ is the ponderomotive phase, $\gamma$ is the electron energy, $a_w$ is the normalized local wiggler amplitude, and $a$ is the normalized vector potential of the radiation field. Further, $\left<.\right>$ indicates an average over the electron bunch. This refractive index envelopes all of the FEL physics contained in the FEL wave equation. However, it is complicated by the presence of the local bunching factor $\left<e^{-i\psi}\right>$, which itself evolves as a function of the radiation field. Information about the bunching factor development must in general be supplemented in some other way, which makes a self-consistent approach using this optical fiber analogy difficult. 

Several approaches have been proposed in the past to make progress towards a self-consistent treatment using the index. In \cite{sprangle1987}, the authors exploited the fact that the bunching factor can be explicitly written in terms of the local field value in the exponential gain regime in the absence of energy spread. The same authors solved the equations using a source-dependent expansion technique which allowed for significant flexibility in the geometries they could study. This approach comes with some drawbacks, however, as it applies only in the exponential gain regime, it neglects the effects of energy spread, and it includes the effect of electron beam emittance only by treating the beam radius as a z-dependent quantity. This is not sufficient, as even in a matched focusing channel where the emittance effects on the electron beam size are cancelled, the emittance still plays a role in the FEL interaction by introducing an angular detuning to the FEL resonance condition. 

The authors of \cite{scharlemann1985} proposed a slightly different method with similar drawbacks. In this case, the transverse laplacian term in the wave equation was taken to be approximately $\nabla_\perp^2E\sim -2k_rE/z_r$ where $z_r$ is the local rayleigh length of the approximately gaussian radiation field. When this simplification is made and the exponential gain regime is assumed, a set of coupled equations relating the FEL power gain length to the mode size allows for a self-consistent propagation of the field through the FEL. The approximation of the transverse laplacian in this way is consistent with assuming the radiation field to have a gaussian transverse dependence, which is in general a good approximation. The drawbacks of this model lie in the assumption that the electron energy profile is uniform, and again an insufficient treatment of emittance effects. 

In the present work we will present a new approximation to the FEL refractive index with the intent to expand on these prior methods in several ways. Our approximation relies on treating the refractive index, and therefore all of the relevant FEL physics, to second-order in the transverse variables. We will show that this approximation couples well to a gaussian ansatz for the radiation field. The limitations and possible extensions of this approximation are discussed later in the paper. This method will apply not just in the exponential gain regime but also in the lethargy regime at the entrance of the undulator. We will also account for both energy spread and emittance in a rigorous way. By removing the explicit assumption of azimuthal symmetry, we will also account for transverse offsets in both the radiation beam and the electron beam. 

The inception of the first x-ray free-electron laser, the LCLS at SLAC, as well as the several FELs that followed it globally, have provided the scientific community with x-ray photons of unprecedented brightness and transverse coherence in ultra-short pulses. In spite of its success, the traditional self-amplified spontaneous emission (SASE) FEL has always suffered from poor longitudinal coherence owing to the fact that the process necessarily starts from noise in the longitudinal phase space. As such, several approaches have been proposed to improve longitudinal coherence. These approaches generally entail seeding the FEL process in some way so that the eventual pulse profile is dominated by a narrow bandwidth seed rather than the noise in the electron beam. 

One such method, which is the focus of a joint ANL-SLAC collaboration, is the cavity-based x-ray free-electron laser (CBXFEL). In this scheme the FEL undulator is wrapped in an optical cavity capable of storing the x-ray beam over many passes. In each pass through the cavity, the radiation beam is frequency-filtered at Bragg mirrors and refocused into the undulator where it is amplified by the FEL gain process. Once the stored power exceeds the effective shot noise power of the electron beam, the clean filtered longitudinal profile becomes dominant resulting in a radiation beam with excellent coherence both transversely and longitudinally. 

Numerical studies of a CBXFEL are, unsurprisingly, extremely expensive with respect to both computing power and time. CBXFEL studies entail all of the usual difficulties associated with numerical studies of FELs with the added difficulty of needing to perform simulations over many passes. This includes both the dozens of simulations of FEL gain in the undulator as well as an equal number of x-ray propagation simulations around the cavity. As such, optimization studies can be unwieldy and slow-going, even when only a single frequency component of the radiation field is considered. 

With these difficulties in mind, we propose here a method by which single-frequency FEL simulations may be greatly sped up using an approximate formalism based on a gaussian ansatz for the radiation field and a simplified treatment of the FEL gain medium, the electron beam, as a quadratic gradient index optical fiber. This numerical method is applicable generally whenever the transverse radiation profile is well-approximated by a gaussian and the input power is large relative to the shot noise, both of which are well-satisfied in the high-gain regime of the CBXFEL: the regenerative amplifier FEL (RAFEL). 

